Performance Analysis of Hardware-Accelerated 10-Bit 4:2:2 Encoding with Split-Frame Encoding for High-Fidelity V-PCC Streaming

Video-based Point Cloud Compression (V-PCC) encodes volumetric data by projecting 3D geometry and texture onto 2D video frames. To prevent spatial distortion and color bleeding during 3D reconstruction, this process requires 10-bit color depth and 4:2:2 chroma subsampling, rather than the standard 8-bit 4:2:0 format. Additionally, capturing high-density dynamic point clouds requires demanding encoding parameters, such as 8K resolution at framerates up to 120 fps. Historically, the lack of 4:2:2 chroma support in older GPU hardware encoders restricted real-time V-PCC to custom Application-Specific Integrated Circuits (ASICs). However, the recent introduction of NVIDIA's Blackwell GPU architecture, featuring on-chip hardware encoders with 10-bit 4:2:2 support, presents an opportunity to shift this workload to general-purpose hardware. This paper investigates the feasibility of such an approach. Using a commercially available Blackwell GPU equipped with four parallel on-die hardware encoders as a testbed, we evaluate the throughput, rate-distortion (RD) performance, and power consumption of 8K 10-bit 4:2:2 HEVC across various Split-Frame Encoding (SFE) configurations. Our results demonstrate that 4-way SFE achieves an encoding throughput of 122 fps, successfully meeting the strict real-time constraints of high-density V-PCC. Although the inability to exploit spatial redundancies across slice boundaries results in a BD-Rate penalty of up to 5%, the measured throughput and power efficiency establish standard, commercial off-the-shelf GPUs as a highly viable baseline for real-time volumetric video streaming.

==> latexmkrc <==
###############################
# Add shell-escape
###############################

$latex = 'latex  %O  --shell-escape %S';
$pdflatex = 'pdflatex  %O  --shell-escape %S';

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

==> rebuttal.tex <==
0468
weakness:No suggestion for how to handle prediction failures effectively.

rebuttal: The contrast failure can be compensated based on the previous frames.  In addition, this problem may result from insufficient training, which can be solved with longer training and a more suitable loss function.

02CE
weakness:Currently, all video contents are compressed prior to be transmitted. Could the authors justify why they do not consider video comrpession in their complete end-to-end transmission system? How does compression affect the performances of the proposed method?

rebuttal: In the paper, we don't consider video compression for simplicity, although our approach can be combined with video compression. In that case,  our proposed prediction will be applied after decoding the streamed video. Video compression causes more delay and image distortion, which is solved by larger timestep prediction and noise-aware training, in which training images originally have compression artifacts. 

1BEB
weakness:what is "t+5" (as tested in the experiments) compared to the streaming latency ?

rebuttal: "t+5" means predicted frame is 5 frames ahead of the current frame. Cityscapes sequence is captured at a framerate of 17Hz. Therefore, "t+5" amounts to 0.29s. 

1AE6(high priority to respond)
weakness:Personally, I feel this work's novelty and contribution are limited and do not meet the ICIP requirements. Extending video interpolation to video prediction is trivial: swap the order of two video frames, and the three training methods are also intuitive. Also, the proposed IFRVP-Fast is just a minor tweak of the original IFRVP: instead of doubling the number of channels, the authors split the input features into two. 
Also, Section 2 Background should be significantly shortened to save room for the authors’ own work instead of details of prior works.

rebuttal: Our main contribution is proposing lightweight network architectures for video prediction that result in better speed-accuracy tradeoffs than DMVFN (CVPR2023 former SOTA). Compared to IFRVP, IFRVP-Fast more aggressively switches the depth of non-linear layers depending on the path. We quantitatively prove the effectiveness and investigate the advantages and disadvantages of our prediction methods through a significant number of experiments. We believe our contribution could be considered eligible for ICIP. 

%Our first main contribution is quantitatively proving the effectiveness and investigating the advantages and disadvantages of our prediction methods through significant amounts of experiments. 
%Our second contribution is proposing an efficient network architecture for video prediction from the viewpoint of parameter efficiency and convergence of the network. Our proposed architecture more aggressively switches the depth of  non-linear layers depending on the path than the original IFRVP. This architecture design results in a better trade-off between speed and accuracy than DMVFN(CVPR2023, former State-Of-The-Art).




0EFC
weakness:1.The paper lacks a detailed discussion on the limitations of the proposed method.  It would be helpful to address potential challenges or scenarios where the method may not perform as effectively.  Additionally, while the relevance of the paper to ICIP is evident, it would be beneficial to further elaborate on how the proposed method contributes to the field of image and video processing.
2. It would be interesting to know if the authors have considered any potential applications beyond video prediction, as well as any plans for future research to address the limitations and further improve the proposed method.

rebuttal: Video prediction has various applications and our method is not limited to any particular usage, although our main goal is to utilize it for low-latency video streaming, as mentioned in Section 2.3.
Currently our method is based only on the video frames. However, our planned future work includes making good use of non-visual information, such as sound in videos and vehicle velocity in autonomous driving.

%1. Since video prediction can be applied variously, we don't specify the usage in a limited area, however, we aim to utilize video prediction for low-latency video transmission as mentioned in section 2.3.
%2. Our method only uses video frames. However, we plan to utilize other information, such as sound in video communication, car velocity in autonomous driving, and the position of robot arms in teleoperation.

We are sorry to say our paper looks not novel. However, even if intuitive, please recognize that classification of three training methods in Fig.3 has not been discussed somehow in the past video prediction research. We also incorporate multiple techniques into the prediction network while keeping real-time performance, and carried out many experiments. 


We sincerely thank all the reviewers for the insightful and supportive comments. We will carefully address the suggestions if our paper is accepted.

Response to reviewer 0468:
Though prediction failure management is not discussed in this paper, we have worked on this topic in the past two years. We think that we should use the predicted video differently according to the application. We can show the predicted video directly for TV conferences and online games, but we might have to limit its usage and only show the predicted video as overlay assistance in critical cases, such as remote surgery and remote driving. For remote control, we can also consider integration with the autonomous control unit at the remote side to avoid operation failures. 

Response to reviewer 02CE:
We did not discuss video compression in this paper as our target is to outperform existing video prediction methods. However, as suggested, we agree that combining with video compression is an important topic, namely compressed-domain video prediction, in addition to prediction from decoded pictures. Note that we have published compressed domain computer vision methods such as J. Liu et al., "Improving Multiple Machine Vision Tasks in the Compressed Domain," ICPR, Aug. 2022.

Response to reviewer 1BEB:
We are sorry for the obscure notation. "t+5" means 5-frame-ahead predicted frame, which corresponds to 0.3 sec future frame in the case of Cityscapes sequence. 

Response to reviewer 1AE6:
Our main contribution is proposing lightweight network architectures for video prediction that result in better speed-accuracy tradeoffs than DMVFN (CVPR2023 former SOTA). The classification of the three training methods shown in Fig. 3 has not been discussed in past works, even if they may look intuitive. We also incorporate multiple techniques into the prediction network while keeping real-time performance, such as in IFRVP-Fast, where we more aggressively switch the depth of non-linear layers depending on the path. We quantitatively and qualitatively prove the effectiveness and investigate the advantages and disadvantages of our prediction methods through a significant number of experiments. We believe this contribution could be considered eligible for ICIP. 

Response to reviewer 0EFC:
1. As suggested, video prediction performance depends on input pictures; it works well for simple pictures like human faces and monotonous motion pictures, but prediction error becomes larger for complicated motion pictures. Therefore, robust video prediction remains the future research, where better prediction and optical flow methods have to be developed.  
2. We think potential applications of video prediction are wide, from TV conferences to autonomous driving, but we also take care of prediction error criticality, as we wrote in response to reviewer 0468. For future research, we consider (1) multi-modal/cross-modal prediction with other sensors, (2) integration with (learned) video compression, and (3) longer video generation. For (1), we published a preliminary paper: Y. Katsuyama et al., "A Predictive Approach for Compensating Transmission Latency in Remote Robot Control for Improving Teleoperation Efficiency", IEEE Globecom, Dec. 2023, where we tried to integrate video and somatic sensors for better prediction.  

